Gravitational Waves and the Galactic Potential

Over the next decade, third-generation interferometers and the space-based LISA mission will observe binaries in galactic centers involving supermassive black holes with millions of solar masses. More precise measurements of more extreme events that probe stronger gravitational fields can have a tremendous impact on fundamental physics, astrophysics, and cosmology. However, at the galactic scale, accretion disks, dark matter halos, and dense populations of compact objects can interact gravitationally with coalescing bodies. The role these astrophysical structures play in the evolution and gravitational-wave signature of binary systems remains largely unexplored and previous studies have often relied on ad-hoc Newtonian approximations. In this thesis, we aim to improve this picture. We study how tidal deformations of matter surrounding black holes can mask off deviations from General Relativity. We also explore the deep connection between light rings -- closed orbits of massless particles -- and the proper oscillation modes of compact objects. We show that independently of the presence of an environment, the light ring controls the late-time appearance of infalling matter to distant observers and how the final black hole formed in a collision relaxes to stationarity. Finally, we develop the first fully-relativistic framework capable of studying gravitational wave emission in non-vacuum environments. We apply it to galactic black-hole binaries surrounded by a dark matter halo and observe the conversion between matter and gravitational waves. This coupling results in significant changes in the energy flux emitted, which could help constrain the properties of galactic matter distributions.

==> Chapters/app_BS.tex <==
%*****************************************
\chapter{Extreme-mass-ratio-inspirals immersed in Scalar Fields}\label{app:BS}
%*****************************************


